PlaneNet: Piece-wise Planar Reconstruction from a Single RGB Image

This paper proposes a deep neural network (DNN) for piece-wise planar depthmap reconstruction from a single RGB image. While DNNs have brought remarkable progress to single-image depth prediction, piece-wise planar depthmap reconstruction requires a structured geometry representation, and has been a difficult task to master even for DNNs. The proposed end-to-end DNN learns to directly infer a set of plane parameters and corresponding plane segmentation masks from a single RGB image. We have generated more than 50,000 piece-wise planar depthmaps for training and testing from ScanNet, a large-scale RGBD video database. Our qualitative and quantitative evaluations demonstrate that the proposed approach outperforms baseline methods in terms of both plane segmentation and depth estimation accuracy. To the best of our knowledge, this paper presents the first end-to-end neural architecture for piece-wise planar reconstruction from a single RGB image. Code and data are available at https://github.com/art-programmer/PlaneNet.

==> cvpr_eso.tex <==
%%
%% This is file `everyshi.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% everyshi.dtx  (with options: `package')
%% 
%% Copyright (C) [1994..1999] by Martin Schroeder. All rights reserved.
%% 
%% This file is part of the EveryShi package
%% 
%% This program may be redistributed and/or modified under the terms
%% of the LaTeX Project Public License, either version 1.0 of this
%% license, or (at your option) any later version.
%% The latest version of this license is in
%%    CTAN:macros/latex/base/lppl.txt.
%% 
%% Happy users are requested to send me a postcard. :-)
%% 
%% The EveryShi package contains these files:
%% 
%%       everyshi.asc
%%       everyshi.dtx
%%       everyshi.dvi
%%       everyshi.ins
%%       everyshi.bug
%% 
%% Error Reports in case of UNCHANGED versions to
%% 
%%                         Martin Schr"oder
%%                         Cr"usemannallee 3
%%                         D-28213 Bremen
%%                         Martin.Schroeder@ACM.org
%% 
%% File: everyshi.dtx Copyright (C) 2001 Martin Schr\"oder
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{everyshi}
         [2001/05/15 v3.00 EveryShipout Package (MS)]
%% \CharacterTable
%% {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%  Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%  Digits        \0\1\2\3\4\5\6\7\8\9
%%  Exclamation   \!     Double quote  \"     Hash (number) \#
%%  Dollar        \$     Percent       \%     Ampersand     \&
%%  Acute accent  \'     Left paren    \(     Right paren   \)
%%  Asterisk      \*     Plus          \+     Comma         \,
%%  Minus         \-     Point         \.     Solidus       \/
%%  Colon         \:     Semicolon     \;     Less than     \<
%%  Equals        \=     Greater than  \>     Question mark \?
%%  Commercial at \@     Left bracket  \[     Backslash     \\
%%  Right bracket \]     Circumflex    \^     Underscore    \_
%%  Grave accent  \`     Left brace    \{     Vertical bar  \|
%%  Right brace   \}     Tilde         \~}
%%
%% \iffalse meta-comment
%% ===================================================================
%%  @LaTeX-package-file{
%%     author          = {Martin Schr\"oder},
%%     version         = "3.00",
%%     date            = "15 May 2001",
%%     filename        = "everyshi.sty",
%%     address         = {Martin Schr\"oder
%%                        Cr\"usemannallee 3
%%                        28213 Bremen
%%                        Germany},
%%     telephone       = "+49-421-2239425",
%%     email           = "martin@oneiros.de",
%%     pgp-Key         = "2048 bit / KeyID 292814E5",
%%     pgp-fingerprint = "7E86 6EC8 97FA 2995 82C3  FEA5 2719 090E",
%%     docstring       = "LaTeX package which provides hooks into
%%                        \cs{shipout}.
%%  }
%% ===================================================================
%% \fi

\newcommand{\@EveryShipout@Hook}{}
\newcommand{\@EveryShipout@AtNextHook}{}
\newcommand*{\EveryShipout}[1]
   {\g@addto@macro\@EveryShipout@Hook{#1}}
\newcommand*{\AtNextShipout}[1]
   {\g@addto@macro\@EveryShipout@AtNextHook{#1}}
\newcommand{\@EveryShipout@Shipout}{%
   \afterassignment\@EveryShipout@Test
   \global\setbox\@cclv= %
   }
\newcommand{\@EveryShipout@Test}{%
   \ifvoid\@cclv\relax
      \aftergroup\@EveryShipout@Output
   \else
      \@EveryShipout@Output
   \fi%
   }
\newcommand{\@EveryShipout@Output}{%
   \@EveryShipout@Hook%
   \@EveryShipout@AtNextHook%
      \gdef\@EveryShipout@AtNextHook{}%
   \@EveryShipout@Org@Shipout\box\@cclv%
   }
\newcommand{\@EveryShipout@Org@Shipout}{}
\newcommand*{\@EveryShipout@Init}{%
   \message{ABD: EveryShipout initializing macros}%
   \let\@EveryShipout@Org@Shipout\shipout
   \let\shipout\@EveryShipout@Shipout
   }
\AtBeginDocument{\@EveryShipout@Init}
\endinput
%%
%% End of file `everyshi.sty'.

